A Monte Carlo Framework for Rendering Speckle Statistics in Scattering Media

We present a Monte Carlo rendering framework for the physically-accurate simulation of speckle patterns arising from volumetric scattering of coherent waves. These noise-like patterns are characterized by strong statistical properties, such as the so-called memory effect, which are at the core of imaging techniques for applications as diverse as tissue imaging, motion tracking, and non-line-of-sight imaging. Our framework allows for these properties to be replicated computationally, in a way that is orders of magnitude more efficient than alternatives based on directly solving the wave equations. At the core of our framework is a path-space formulation for the covariance of speckle patterns arising from a scattering volume, which we derive from first principles. We use this formulation to develop two Monte Carlo rendering algorithms, for computing speckle covariance as well as directly speckle fields. While approaches based on wave equation solvers require knowing the microscopic position of wavelength-sized scatterers, our approach takes as input only bulk parameters describing the statistical distribution of these scatterers inside a volume. We validate the accuracy of our framework by comparing against speckle patterns simulated using wave equation solvers, use it to simulate memory effect observations that were previously only possible through lab measurements, and demonstrate its applicability for computational imaging tasks.

==> applications_o.tex <==
\section{Applications}\label{sec:applications}

As argued above speckle correlations have applications in   several computational imaging tasks. In this section we demonstrate a few examples. 



 \begin{figure}[!t]
        \begin{center}\begin{tabular}{c}
                        \includegraphics[width= 0.2  \textwidth]{figures/CovvsInt.eps}
                \end{tabular}\vspace{-0.5cm}
        \end{center}
        \caption{\small{ Phase function discrimination: The error in explaining measurements with a wrong phase function, as a function of the anisotropy parameter $g\in[-1, 1]$ of a  Henyey-Greenstein phase function. The correlation provides a sharper, less ambiguous minimum around the true value, when compared to intensity measurements. }  }\label{fig:corr-reconst}
\end{figure}


\subsection{Validating the memory effect of speckles}

The memory effect of speckles is an active research area in optics.  For thin scattering media,  a light-emitting object hidden behind a scattering layer is numerically reconstructed from its transmitted speckle pattern~\cite{Katz2014,Bertolotti2012}, using speckle  autocorrelation. As a result of the memory effect, speckle images produced by different light positions are a shifted version of each other, hence the speckle auto-correlation is equivalent to the  auto-correlation of source positions.  Another approach that is valid when the transmission matrix is available   (e.g., by placing a point source or detector behind the scattering
layer)
 is to actively modulate  the incident wavefront and focus inside turbid media~\cite{Mosk2012,Nixon2013}.  The memory effect plays again an important task as if one measured the modulation pattern at one position (e.g. by recording a flurecent source), a shift/tilt of the same pattern can be used at nearby points~\cite{GenOptMemory17,Vellekoop:10}. 

As all these approach are relying on the memory effect, it is crucial to understand at what range of illumination and viewing configurations we can indeed expect a high correlation between speckles under different illumination directions.

There have been multiple attempts~\cite{GenOptMemory17,BERKOVITS1994135,Fried:82} to derive close form formulas for speckle correlations but the complexity of the problem required various assumptions that limits the approximation accuracy and the applicability of such formulas. The main theoretical result~\cite{feng1988correlations,Akkermans07} is a formula derived under diffusion assumptions that is valid for materials that are thick enough so that light scatters  multiple times, stating
 \BE\label{eq:corr-diffusion}
 C(\theta)\approx\frac{(k \theta L)^2 }{sinh^2(k \theta L)}
 \EE
where $\theta$ is the angle between illumination and viewing directions, $L$ is the material thickness, $k=2\pi/\lambda$ is the wave number, and $ C(\theta)$ is the correlation between intensity images (rather than complex fields) $I^\ind_\outd$ and $I^{\ind+\theta}_{\outd+\theta}$.
 The correlation of \equref{eq:corr-diffusion} decays to zero exponentially fast as soon as $k\theta L>1$, hence the angular range at which the memory effect is valid is proportional to $1/(kL)$. While \equref{eq:corr-diffusion} is derived assuming a high optical depth, or a large number of scattering events, empirical observations  suggest that in practice the memory effect is valid through a much wider range. A few parameters that can increase its range are (i) when the average number of scattering events is lower than the diffusive regime, (ii) absorption, (iii) forward scattering phase functions. Forward scattering is particularly important in practice as tissue is known to be highly forward scattering and is usually described by anisotropy parameters $g\in [0.85-0.95]$.  Given the luck of analytic formulas and the practical importance of the problem, there have been multiple attempts to empirically  measure the range of the memory effect of materials of interest in the lab~\cite{Schott:15,Yang:14,mesradi:hal-01316109}.
  


An advantage of our technique is that we can compute the expected correlations directly, bypassing the complex lab setup.  Correlation is computed as a function of simple material parameters such as thickness, $\extCoff$, $\sctCoff$ and phase function. In \figref{} we show numerical calculations of the expected correlation as a function of angle.   In \figref{}(a) we use a forward scattering configuration, isotropic phase function $g=0$ and vary the mean free path. For a high optical depth the correlation computed by our MC approach agrees with the theoretical formula of \equref{eq:corr-diffusion}, and as the optical depth decreases (mean free path increases) the range of the memory increases. In \figref{}(b)  we kept the density fixed and varied the anisotropy of the phase function. As previous empirical observations report~\cite{}, our MC evaluation predicts that the memory effect range increases with the anisotropy parameter $g$.  In \figref{}(c) we evaluated a backscattering configuration for fixed $g$ and $\extCoff$, but varied albedo. As expected one can observe that the memory effect is better with absorbing materials.
In \figref{}(d) we considered the specific case of chicken breast tissue that was imaged  by~\cite{}. Using the mean free path and $g=0.96$ values they report we simulated the exact same material thickness reported in this work and predicted the range of the memory effect, comparing it with the reported empirical measurements.

Note that our MC algorithm computes correlations of complex fields while \equref{eq:corr-diffusion} evaluates intensity correlations. However, field covariances can be easily converted to intensity covariances as $2|C^{\inp_1,\inp_2}_{\snsp_1,\snsp_2}|^2$.


To demonstrate an application of speckle correlation we reproduced the algorithm of ~\cite{Katz2014}. This algorithm attempts to recover a set of incoherent light sources located behind a scattering layer. Due to the memory effect the auto-correlation of the speckle image should be equivalent to the auto-correlation of position of light sources. Thus, given the seemingly random speckle image one can recover the position of light sources behind it by applying a phase retrieval algorithm~\cite{}.
In \figref{} we show the result of this reconstruction applied on speckle images rendered with Algorithm \ref{alg:MCfield}. We have  repeated this for materials with a few optical depths. As we have selected the position of the hidden sources to be a bit outside the range of the memory effect, for the thick materials only the central sources were recovered. As we reduced the average number of scattering events the memory effect range increases and the reconstruction improves.
  
 




==> figure-example-setup.tex <==
\begin{figure*}[t]
\centering
 \begin{tabular}{@{}c@{}c@{}}
 \begin{tabular}{@{}c@{}}
 \includegraphics[height=0.34\linewidth]{figures/example-setup/setupSingleIncident}\\\begin{footnotesize}(a) Setup with one illuminator
\end{footnotesize}\end{tabular}&
  \begin{tabular}{@{}c@{}c@{}c@{}}
  \includegraphics[width=0.15\linewidth]{figures/example-setup/specklesOneSource1}&
  \includegraphics[width=0.15\linewidth]{figures/example-setup/mudiff_cov1_1}&
  \includegraphics[width=0.15\linewidth]{figures/example-setup/diag1_1}\\
  \begin{footnotesize}(b) Sampled field 1\end{footnotesize}& \begin{footnotesize}(d) Wave solver cov\end{footnotesize} &\begin{footnotesize}(f) Diagonal plot from (d,e)\end{footnotesize}\\
  \includegraphics[width=0.15\linewidth]{figures/example-setup/specklesOneSource2}&
  \includegraphics[width=0.15\linewidth]{figures/example-setup/mc_cov1_1}&
  \includegraphics[width=0.15\linewidth]{figures/example-setup/line1_1}\\
   \begin{footnotesize}(c) Sampled field 2\end{footnotesize}& \begin{footnotesize}(e) MC covariance\end{footnotesize} &\begin{footnotesize}(g) Raw plot from (d,e)\end{footnotesize}\\
\end{tabular}\\
 \begin{tabular}{@{}c@{}}\includegraphics[height=0.34\linewidth]{figures/example-setup/setupTwoIncidents}\\\begin{footnotesize}(h) Setup with two illuminations\end{footnotesize}
\end{tabular}&
  \begin{tabular}{@{}c@{}c@{}c@{}}
   \includegraphics[width=0.15\linewidth]{figures/example-setup/specklesTwoSources1}&
  \includegraphics[width=0.15\linewidth]{figures/example-setup/mudiff_cov1_2}&
  \includegraphics[width=0.15\linewidth]{figures/example-setup/diag1_2}\\
  \begin{footnotesize}(i) Sampled field 3\end{footnotesize}& \begin{footnotesize}(k) Wave solver cov\end{footnotesize} &\begin{footnotesize}(m) Diagonal plot from (k,l)\end{footnotesize}\\
  \includegraphics[width=0.15\linewidth]{figures/example-setup/specklesTwoSources2}&
  \includegraphics[width=0.15\linewidth]{figures/example-setup/mc_cov1_2}&
  \includegraphics[width=0.15\linewidth]{figures/example-setup/line1_2}\\
   \begin{footnotesize}(j) Sampled field 4\end{footnotesize}& \begin{footnotesize}(l) MC covariance\end{footnotesize} &\begin{footnotesize}(n) Raw plot from (k,l)\end{footnotesize}\\
\end{tabular}
 \end{tabular}
 \caption{{\bf Simulating speckle and their statistics.} (a) Consider a rectangular scattering volume illuminated by a plane wave and a scattered field  sensed by collinear sensors. For each scatterer instantiation we solve the wave equation~using the package of \cite{mudiff} and compute the scattered field, shown in (b,c). Different scatterer positions lead to different high-fluctuation speckle fields. The empirical  covariance of multiple fields obtained with the wave solver is demonstrated in (d), and is closely matched by the covariance computed directly by our Monte Carlo algorithm (e). To demonstrate the good agreement we overlay a diagonal plot (f) and a row plot (g). The diagonal of the speckle covariance is equivalent to intensity images computed by standard incoherent intensity MC algorithms.  In the lower row (h) we consider a situation where the same scatterer instantiation is illuminated by two mutually coherent waves, highlighting that despite their semi-random structure speckles have strong statistical properties. In particular, the memory effect of speckles: when the same set of scatterers is illuminated by two mutually coherent waves the resulting speckle patterns are shifted versions of each other (i-j). This also implies that the covariance of the speckle fields (k) generated by two illumination directions has a shifted diagonal, where the diagonal offset corresponds to fields shift. Our Monte Carlo algorithm is physically correct and captures all such statistics, while having a computational complexity several orders of magnitude smaller than the wave equation solver.}  \label{fig:example-setup}    
\end{figure*}


==> figure-phantom-size-diag-width.tex <==
\begin{figure*}[t]
%\begin{tabular}{c}
\centering
%
%
\hspace{-4cm}
\subfloat{\makebox[0.24\textwidth][c]{$10\times10$}}
\subfloat{\makebox[0.22\textwidth][c]{$20\times20$}}
\subfloat{\makebox[0.22\textwidth][c]{$50\times50$}}
\\
	\subfloat{\raisebox{2cm}{\rotatebox[origin=t]{90}{MC}}}\hspace{0.5cm}
	\subfloat{\label{fig:fig3_mc_mfp_10}\includegraphics[width=0.23\textwidth]
		{figures/phantom-size-diag-width/fig3_mc_mfp_10}}
	\subfloat{\label{fig:fig3_mc_mfp_20}\includegraphics[width=0.23\textwidth]
		{figures/phantom-size-diag-width/fig3_mc_mfp_20}}
	\subfloat{\label{fig:fig3_mc_mfp_50}\includegraphics[width=0.23\textwidth]
		{figures/phantom-size-diag-width/fig3_mc_mfp_50}}\hfill
	\subfloat{\label{fig:fig3_line}\includegraphics[width=0.22\textwidth]
		{figures/phantom-size-diag-width/fig3_line}}
\\ \vspace{-0.2cm}
        \centering
\subfloat{\raisebox{2cm}{\rotatebox[origin=t]{90}{Wave Solver}}}\hspace{0.5cm}
\subfloat{\label{fig:fig3_mudiff_mfp_10}\includegraphics[width=0.23\textwidth]
	{figures/phantom-size-diag-width/fig3_mudiff_mfp_10}}
\subfloat{\label{fig:fig3_mudiff_mfp_20}\includegraphics[width=0.23\textwidth]
	{figures/phantom-size-diag-width/fig3_mudiff_mfp_20}}
\subfloat{\label{fig:fig3_mudiff_mfp_50}\includegraphics[width=0.23\textwidth]
	{figures/phantom-size-diag-width/fig3_mudiff_mfp_50}}\hfill
\subfloat{\label{fig:fig3_lineZoomed}\includegraphics[width=0.22\textwidth]
	{figures/phantom-size-diag-width/fig3_lineZoomed}}
%\end{tabular}
\comment{
	\begin{tabular}{c}
	\subfloat[]{\label{fig:fig3_line}\includegraphics[width=0.27\textwidth, height=0.4\textwidth]
		{figures/phantom-size-diag-width/fig3_line}}
\end{tabular}}
  \caption{Target size and speckle width. We compare the result of our MC algorithm and a wave solver for three different target sizes (O.D.=1) using zero degree plane wave illumination and viewing $360^{\circ}$ in the far field. Notice how the width of the diagonal decreases with increasing target size. Hence, the width of speckles decreases when increasing target size. In the last column we show a plot of the marked dashed line. The increasing width can be clearly seen. }  
   \label{fig:phantom-size-diag-width}        
\end{figure*}

